Reproducing the results for NICER observation of PSR J0030+0451

NASA's Neutron Star Interior Composition Explorer (NICER) observed X-ray emission from the pulsar PSR J0030+0451 in 2018. Riley et al. reported Bayesian parameter measurements of the mass and the star's radius using pulse-profile modeling of the X-ray data. This paper reproduces their result using the open-source software X-PSI and publicly available data within expected statistical errors. We note the challenges we faced in reproducing the results and demonstrate that the analysis can be reproduced and reused in future works by changing the prior distribution for the radius and the sampler configuration. We find no significant change in the measurement of the mass and radius, demonstrating that the original result is robust to these changes. Finally, we provide a containerized working environment that facilitates third-party reproduction of the measurements of mass and radius of PSR J0030+0451 using the NICER observations.

==> sec-reanalysis.tex <==
\section{REPRODUCING THE ANALYSIS}\label{sec:re-analysis}

For their analysis, Riley \textit{et al.} used \textit{X-PSI} --- an open-source software developed to analyze X-ray pulse profile data. It is written primarily in Python 2.7, with additional Cython support. It simulates X-ray emission from hotspots on a rotation-powered pulsar and uses it for Bayesian analysis of observed data. For posterior sampling purposes, it uses the nested sampling algorithm \texttt{MULTINEST} \cite{ferozMultiNestEfficientRobust2009}. 

Riley \textit{et al.} used \textit{X-PSI} v0.1 to analyze PSR J0030+0451. Since v0.1 of \textit{X-PSI}, substantial changes and upgrades have been made to the code and its documentation, making it difficult for a user to write configuration files from scratch to replicate an analysis done with the previous code version. 

However, Riley \textit{et al.} also released a Zenodo repository\footnote{\url{https://doi.org/10.5281/zenodo.5506838}} that contains the event data, the configuration files for \textit{X-PSI} v0.1, the submit scripts for the job, the output files of the job, and the files containing the posterior samples for each analysis. This release makes it fairly straightforward for anyone who wants to reproduce the original analysis, as long as they have installed the software and its dependencies and have enough computational resources. The repository comes with a \texttt{README.txt} that briefly describes each file and its use. For our analysis, we used the configuration files from the repository, only changing the paths to the input data and output files wherever necessary.

The biggest challenge came in fully utilizing the parallelization capabilities of \textit{X-PSI}. The analysis involves $\mathcal{O}(10^8)$ likelihood evaluations each taking $\mathcal{O}(1)$ sec of evaluation time. One such step involves simulating hotspots on the star's surface, ray tracing the radiation to include relativistic effects, and creating an instance of the X-ray pulse that a distant observer would detect, making likelihood evaluation the most computationally expensive. Finishing the analysis within a reasonable time is possible if one can evaluate the likelihood values in parallel using multiple CPUs. The sampler \texttt{MULTINEST} used by \textit{X-PSI} is parallelized and is compatible with Message Passing Interface (MPI). However, to include MPI into our workflow that has everything installed within containers was a challenging task. Please see the next section for the workflow details and how this problem was resolved.

Another obstacle in reproducing the original results was postprocessing and plotting the output of the Bayesian analysis. Although the Zenodo repository had all the configuration files and submitted scripts to start the analysis, the postprocessing and plotting scripts were absent. The scripts were necessary to produce a figure that was identical to the figure that was published. The documentation of \textit{X-PSI} describes the postprocessing module of the software. However, the documentation describes the use of v0.5 of \textit{X-PSI}, which is backward incompatible with v0.1 used in the original analysis. We found that the postprocessing module of \textit{X-PSI} failed to process the output files from \texttt{MULTINEST}. Instead, we used the postprocessing modules and scripts from PyCBC Inference~\cite{Biwer:2018osg}--a Python toolkit for Bayesian analysis of gravitational-wave signals--to plot all the posteriors. We converted the \texttt{.dat} files produced by the \texttt{MULTINEST} sampler into PyCBC-readable \texttt{.hdf} files and used the \texttt{pycbc\_plot\_posterior} script on these files. This emphasizes the importance of releasing the source code used in the original analysis, including the postprocessing and the plotting scripts. 

%On visual inspection of the posteriors plotted from the output files from the Zenodo repository, we find that they are the same as those plotted in Figure 19 of Riley \textit{et al.} 


